Radiochromic Film Dosimetry for VHEE and UHDR: Considerations for the CLEAR Facility and Comparisons with Alanine, RPL and Dosimetry Phantoms

Radiochromic films (RCFs) offer valuable two-dimensional dosimetry capabilities with a conceptually simple operating principle that requires minimal investment, making them particularly suitable for very high energy electron (VHEE) FLASH dosimetry where dosimetry standards are currently lacking. However, achieving high-accuracy measurements with RCFs presents significant practical challenges. Without the standardised protocols that ensure reliable outcomes across applications and facilities, knowledge of RCF behaviour becomes essential. This paper identifies common sources of error in RCF preparation, scanning, and processing while proposing specific mitigation strategies to improve accuracy and efficiency. Using our optimised RCF protocol at the CLEAR facility, we demonstrate relative agreement within 5% compared to alanine dosimeters when measuring Gaussian VHEE beams, establishing a foundation for reliable dosimetry in these advanced radiotherapy applications.

==> RCF/old/Films.tex <==



\section{Film Calibration}
The thickness of the active layer will vary slightly between different production lots. It is thus important to characterize each batch under reference conditions in order to establish their response over a range of doses. All calibration curves herein have been obtained by irradiating a set of films at the eRT-6 electron linac at CHUV in Lausanne. By positioning the films in front of an ionization chamber behind \todo{x cm} of solid water, one ensure a uniform dose distribution across the film as well a direct dose measurement to link with the resulting darkening. A set of doses are chosen within the dynamic range of the film in question in geometric progression \todo{why?}, with a minimum of two films per dose-step.

As the optical density of the films increases with increased exposure before reaching a saturation outside of their dynamic range, it is recommended to subsequently fit the calibration curve to a polynomial function of the form 

\begin{equation}
    OD_x(D) = -\mathrm{log}\left(\frac{a+bD}{D-c}\right)
    \label{eq:calib_curve}
\end{equation}

 where $OD_x(D)$ is the optical density of the film in scanner channel $x$ at dose $D$, and $a$, $b$, $c$ are the equation parameters to be fitted. This type of function has the same rational behaviour, and fewer calibration points are thus needed in order to obtain a good fit. It is also easy to invert in order to determine the dose as a function of optical density. 
 A typical case would use 6-8 points (including unexposed film) with the doses in geometric progression \cite{ebt3}. 

 The optical density for a given channel $x$ can be calculated by 

 \begin{equation}
     OD_x=-\mathrm{log}\left(\frac{PV_x}{65535}\right)
     \label{eq:ODx}
 \end{equation}

 where $PV_x$ is the pixel value for channel $x$ and 65535 is the RGB color space for a 16 bit scanner.

 Due to the darkening of films over time, it is good practice to always subtract the background by using an unirradiated reference film as baseline. This is done by subtracting the optical density of the background $OD_{x,0}$ from the optical density of the exposed film $OD_{x,exp}$. In this case Equation \ref{eq:ODx} takes the form

 \begin{equation}
     OD_{x,net}=OD_{x,exp}-OD_{x,0}=-\mathrm{log}\left(\frac{PV_{x,exp}}{PV_{x,0}}\right)
     \label{eq:ODx_net}
 \end{equation}


\section{Image Processing}

  
\subsection{Filtering}

\subsection{Single Channel Methods}
Using the marker dye feature is not mandatory as dosimetry can be done using a single color channel. The manufacturer suggests using the the red channel, as the red light component is closest to the peak absorbance wavelength, giving a better response \cite{mdv3}. However, several sources report on using the green channel \cite{Santos2017QuantificacaoIntra-Operatoria}. Ultimately the choice will depend on the optical density of the film of interest, and which of the three calibration curves are more sensitive to changes in this region. For films exposed to transversally uniform beams, this may be straight forward. However, for beams exhibiting an e.g. Gaussian distribution, one would either have to optimize by using different curves for different parts of the film, or use the one which exhibits the overall highest sensitivity for the entire range.

Based on the established calibration factors for the channel $x$ and film batch in question, the dose may be calculated by combining Equations \ref{eq:calib_curve} and \ref{eq:ODx_net}

\begin{equation}
    D(OD_{x,net})=\frac{a-c\cdot e^{-OD_{x,net}}}{e^{-OD_{x,net}}-b}=\frac{a-c\cdot \left(\frac{PV_{x,exp}}{PV_{x,0}}\right)}{\left(\frac{PV_{x,exp}}{PV_{x,0}}\right)-b}
\end{equation}


\todo{Why?}

\subsection{Multichannel Methods}
The multichannel method allows for the separation of the scanned signal into one part that is dose-dependent and another part that is dose-independent
and enables the correction of a variety of disturbances in the digitized image including thickness differences of the film's active coating as well as scanner related artifacts \cite{micke_multichannel}. 

The active layer also contains a yellow marker dye which enables non-uniformity correction through multi-channel dosimetry and limits their sensitivity to UV and visible light.  

Due to the chromatic nature of GAFChromic film, there is no clear color saturation point. This is an advantage when FilmQAPro Pro software is used for the dosimetry analysis, since the use of the three available color channels effectively extends the dynamic range of the film. However, increasingly shallow slopes of the EBT3 response curves at doses >10 Gy may lead to increased dose uncertainty in this high dose region. As seen in Figure 2, EBT-XD film provides steeper slopes of the red and green response functions  than EBT3 at higher doses and is therefore more desirable for measurements at doses >10 Gy \cite{ebt3}

This provides the ability to compare
dose measurement results from three color channels with the key advantage of
establishing the consistency of these dose values. A poor correspondence of the values
(>4%) equates to substantial dose uncertainty and points towards faulty application of
the protocol, whereas high consistency of the dose values builds confidence in the
measurement results. Dose consistency of better than 2% between the color channels
should be routinely achievable and frequently the results should be better than 1%.
Follow the simple instructions closely and you will find you can rely on radiochromic film
to provide absolute dose measurement that is consistent and dependable \cite{film_protocol}.


\section{Sources of error}
Santos reported on uncertainties between 0.69\% and 0.84\% in the dose calculation from EBT-3 films exposed to 10 to 15 Gy in vivo. 
\cite{Santos2017QuantificacaoIntra-Operatoria}

\subsection{Effect on beam}
\subsection{Time of scan}
\subsection{AOI selection}
\subsection{Film Handling}
Finger prints same film without fp and with fp for 10 films
temperature: frozen to heated for 10 films
light exposure
\subsection{Scanner errors}
Several sources state the importance of having properly warmed up the scanner before scanning films in order to limit scanner-related errors in the film processing. Some film dosimetry protocols suggest that 3-5 scans of the entire scanning area in transmission mode is sufficient \cite{Santos2017QuantificacaoIntra-Operatoria}. 

Cold scanner - cold vs warm scan? evolution, 5 series? 
dust particles
scan several times (3-5) average? 
multiscanning effects? (clean film, scan e.g. 50 times. See difference?
scanner position
orientation, quantify

\section{Protocol for Film Dosimetry}

==> figures/old/confetti.tex <==
\subsection{RCF Confetti}
\label{sec:confetti}

\begin{figure}[htb!]
    \centering
    %\begin{subfigure}[b]{0.45\linewidth}
     %    \centering
     \includegraphics[width=\linewidth]{figures/confetti_holder.png}
         %\caption{A robot holder with an RCF positioned upstream of an eppendorf tube containing 5 smaller pieces of RCF.}
         %\label{fig:confetti_holder}
     %\end{subfigure}
     %\begin{subfigure}[b]{0.45\linewidth}
     %    \centering
     %    \includegraphics[width=\linewidth]{figures/Hex_phantom_holder2.png}
     %    \caption{The structure of the 3D printed dosimetric phantom.}
     %   \label{fig:confetti}
     %\end{subfigure}
     
    \caption{Right: The robot holder with an RCF positioned upstream of an eppendorf tube containing 5 smaller pieces of RCF.}
    \label{fig:confetti_setup}
\end{figure}


==> figures/old/monitor.tex <==




%\usetikzlibrary{arrows,arrows.meta}
\usetikzlibrary{calc}
\usetikzlibrary{math} % for \tikzmath
\usetikzlibrary{angles,quotes} % for pic (angle labels)
\tikzset{>=latex} % for LaTeX arrow head
\contourlength{1.6pt}
\usetikzlibrary{decorations.pathreplacing} % for curly braces
\usetikzlibrary{shapes.geometric,shadings}
\usetikzlibrary{shapes,shadows,arrows,positioning,graphs}
\usetikzlibrary{fadings,decorations.text}
\tikzfading[name=fade inside, inner color=transparent!90, outer color=transparent!40]



 

\tikzstyle{vector}=[->,very thick,myblue,line cap=round]
\tikzstyle{cone}=[thin,blue!50!black,fill=blue!50!black!30,fill opacity=0.8]
\tikzstyle{textbf} = [font=\bfseries]

\begin{figure}

    \begin{center}
        \begin{adjustbox}{max height=.4\textheight, center, width=.3\textwidth}
            % Test setup

            \begin{tikzpicture}[x={(1cm,-0.5cm)}, y={(1cm,0.5cm)}, z={(0cm,1.5cm)}, scale=3.5,
                %Option for nice arrows
                >=stealth, %
                inner sep=0pt, outer sep=2pt,%
                axis/.style={thick,->},
                wave/.style={thick,color=#1,smooth},
                kapton/.style={fill=brown!80!red, opacity=0.7},
                holder/.style={fill=green!30!white!60!black, opacity=0.3},
                elps/.style={ellipse,minimum width=1cm,minimum height=3cm}, 
                circ/.style={circle, minimum width=2cm,minimum height=2cm, rotate around x=45}, 
                screen/.style={fill=yellow!80!brown, opacity=0.7},
                pipe/.style={ellipse,minimum size=4cm}, 
                beampipe/.style={fill=black!50!white, opacity=0.7},
                mirror/.style={fill=black!50!white, opacity=0.8}, 
                beam/.style={fill=red!70!white,red!70!white, opacity=0.8}, 
                light/.style={fill=blue!60!white,blue!60!white, opacity=0.8}
            ]
                
            % Colors
                \colorlet{darkgreen}{green!50!black}
                \colorlet{lightgreen}{green!80!black}
                \colorlet{darkred}{red!50!black}
                \colorlet{lightred}{red!80!black}
                \colorlet{lightblue}{blue!60!white}
                \colorlet{mygreen}{green!40!white}
                \colorlet{beamred}{red!70!white}
                \colorlet{steelgrey}{black!50!white}

                \pgfmathsetmacro{\WPstart}{10} %start of water phantom
                \pgfmathsetmacro{\cubex}{4} %length of water phantom
                \pgfmathsetmacro{\cubey}{2} %width of water phantom
                \pgfmathsetmacro{\cubez}{2} %height of water phantom

                \pgfmathsetmacro{\Hstart}{2} %start of screen holder
                \pgfmathsetmacro{\Hx}{4} %length of screen holder
                \pgfmathsetmacro{\Hy}{3} %width of screen holder
                \pgfmathsetmacro{\Hz}{3} %height of screen holder
                
                
                % Frame
                \coordinate (O) at (0, 0, 0);
            
                %\draw[thick,dashed] (-2,0,0) -- (O);

                %----------------COORDINATE AXES---------------------
                %\draw [thick,dashed,shorten >=2pt] (0,0,0) -- (5,0,0);
                \draw[ultra thick,->] (O) -- (6,0,0) node[anchor=north west]{z};
                \draw[ultra thick,->] (O) -- (0,2,0) node[anchor=south west]{x};
                \draw[ultra thick,->] (O) -- (0,0,2) node[anchor=north east]{y};
            
                %-------------BEAM PIPE----------------
            
                \pgfmathsetmacro{\pipex}{4} %length of beam pipe
                \pgfmathsetmacro{\piper}{0.7} %radius of beam pipe

                

                
                %------BEAM CONE IN AIR--------            
                \node[elps,scale=.2, fill=beamred](n1)at(0,0,0){}; %start of truncated cone
                \node[elps, scale=.5, fill=beamred](n2)at(2,0,0){}; %end of truncated cone
                \draw[beam] (n1.92)--(n2.{92})--(n2.{268})--(n1.268)--cycle; 
                
                %\node[scale=.2,draw, fill=beamred, opacity=.8,elps] (n1)at(\pipex,0,0){};

                 \draw[holder] (\Hstart,.5*\Hy, -.5*\Hz) -- ++(.2*\Hx,0,0) -- ++(.8*\Hx,0,\Hz) -- ++(-\Hx,0,0) node [opacity=1,text=black, above=1cm, sloped, at start, text width=2cm]{OTR} node [opacity=1,text=black, above=1cm, sloped, at end, text width=2cm]{YAG} -- cycle ; %holder right face
                 
                 
                 %YAG
                \draw[screen, opacity=0.5] (\Hstart,.5*\cubey, .5*\cubez) -- ++(0,0,-\cubez) -- ++(0,-\cubey,0) -- ++(0,0,\cubez) -- cycle; %yag\
                \node[scale=.5,draw, fill=beamred, opacity=.8,elps](n2)at(\Hstart,0,0){}; %beam on screen

                 
                 %BEAM CONE IN HOLDER
                \node[elps,scale=.5, fill=beamred](n1)at(\Hstart,0,0){}; %start of truncated cone
                \node[elps, scale=.85, fill=beamred](n2)at(\Hstart+.6*\Hx,0,0){}; %end of truncated cone 
                \draw[beam] (n1.92)--(n2.{92})--(n2.{268})--(n1.268)--cycle;       
                \node[scale=.85,draw, fill=beamred, opacity=0.8, elps] (n2)at(\Hstart+.6*\Hx,0,0){}; %beam front

                %LIGHT CONE IN HOLDER
                \node[elps,scale=.5, fill=lightblue, align=center](n1)at(\Hstart,0,0){}; %start of truncated cone
                \node[elps, scale=.85, fill=lightblue](n2)at(\Hstart+.6*\Hx,0,0){}; %top end of truncated cone 
                \draw[light] (n1.south)--(n2.south)--(n2.north)--(n1.north);%--cycle;       

                

                %HOLDER
                \draw[holder] (\Hstart,.5*\Hy, .5*\Hz)  -- ++(\Hx,0,0) -- ++(0,-\Hy,0) -- ++(-\Hx,0,0) -- cycle; %top face
                %node [opacity=1,text=black, above=1cm, sloped, near end, text width=4cm]{Kapton window}; %top face
                %\draw[holder] (\Hstart+\Hx,.5*\Hy, .5*\Hz) -- ++(0,0,-\Hz) -- ++(0,-\Hy,0) -- ++(0,0,\Hz) -- cycle; %front face\
               
                \draw[holder] (\Hstart,.5*\Hy, -.5*\Hz) -- ++(.2*\Hx,0,0) -- ++(0,-\Hy,0) -- ++(-.2*\Hx,0,0) -- cycle; %bottom face
                
                \draw[holder] (\Hstart,-.5*\Hy, -.5*\Hz) -- ++(.2*\Hx,0,0) node(base){} -- ++(.8*\Hx,0,\Hz) -- ++(-\Hx,0,0) -- cycle; %left face
                
                
                %BEAM SIZE INDICATORS
                \draw[ultra thick, ->] (\Hstart, 0,1) -- (\Hstart, 0, 0.3)
                node [above=.5cm, near start]{\textsigma$\mathrm{_y}$};
                \draw[ultra thick, <-] (\Hstart, 0.,-0.3) -- (\Hstart, 0, -1);

                \draw[ultra thick, ->] (\Hstart, 1,0) -- (\Hstart, 0.3, 0)
                node [above=.5cm, near start]{\textsigma$\mathrm{_x}$};
                \draw[ultra thick, <-] (\Hstart, -0.3,0) -- (\Hstart, -1, 0);

                \coordinate (joint) at (\Hstart+.2*\Hx,-.5*\Hy, -.5*\Hz);
               
                
                \draw[ultra thick, <->] (\Hstart+2, -4,0) -- (\Hstart+\Hx+1.5, -4, 0)
                node [below=1 cm, sloped, midway]{72 mm};


                
                

                %CAMERA

                \pgfmathsetmacro{\camHeight}{5} %start of water phantom
                \pgfmathsetmacro{\camX}{1.5*\Hx}
                \pgfmathsetmacro{\camY}{-0.5*\Hy}

                \node [] at (\camX+2,\camY,\camHeight+0.6){CAMERA};

                %LIGHT CONE TO CAMERA
                \node[elps, scale=.85, fill=lightblue](n1)at(\Hstart+.6*\Hx,0,0){};%start of truncated cone
                \node[elps, scale=.85, fill=lightblue](n2)at(\camX,\camY,\camHeight){}; %top end of truncated cone 
                \draw[light] (n1.west)--(n2.west)--(n2.east)--(n1.east);%--cycle;       
                \node[scale=.85,draw, lightblue, fill=lightblue, elps] (n3)at(\camX,\camY,\camHeight){}; %light front
                \node[scale=.85,draw, fill=lightblue, elps] (n2)at(\Hstart+.6*\Hx,0,0){}; %light front
                \draw[mirror] (\Hstart+.2*\Hx,-.5*\Hy, -.5*\Hz) -- ++(.8*\Hx,0,\Hz) node(otr){} -- ++(0,\Hy,0) -- ++(-.8*\Hx,0,-\Hz) -- cycle; %back face
                \node[elps,scale=.85, fill=beamred, opacity=0.8](n1)at(\Hstart+.6*\Hx,0,0){}; %start of truncated cone
                \node[elps, scale=.85, fill=beamred, opacity=0.8](n2)at(\Hstart+.9*\Hx,0,0){}; %end of truncated cone 
                \draw[beam] (n1.92)--(n2.{92})--(n2.{268})--(n1.268)--cycle;       
                \node[scale=.85,draw, beamred, fill=beamred, opacity=0.8, elps] (n2)at(\Hstart+.9*\Hx,0,0){}; %beam front

                \filldraw[black!85] (\camX,\camY,\camHeight) circle (0.75);
                \draw [darkgray] (\camX,\camY, \camHeight) circle (0.1);
                \shade [ball color=white,path fading=fade inside] (\camX,\camY, \camHeight) circle (0.0975);
                \draw [gray] (\camX,\camY, \camHeight) circle (0.25);
                \draw[] (\camX,\camY, \camHeight) circle (0.3);
                \draw [darkgray] (\camX,\camY, \camHeight) circle (0.375);
                \shade [ball color=white,path fading=fade inside] (\camX,\camY, \camHeight) circle (0.6225);
                \draw [darkgray,thick] (\camX,\camY, \camHeight) circle (0.625);
                \draw [thick] (\camX,\camY, \camHeight) circle (0.675);
                \begin{scope}
                    \clip (\camX,\camY, \camHeight) circle (0.875);
                    \foreach \i in {8,...,10,11} \shade [ball color=white!85!blue, blend mode=hard light, opacity=1] (135:{1.3*(10-\i}) circle ({0.13*\i});
                    \shade [ball color=white!85!blue, shading angle=0, blend mode=hard light, opacity=1] (\camX,\camY, \camHeight) circle (0.65);
                  \end{scope}

                 
                \pic [draw, <->, "45$^\circ$", angle eccentricity=1.5, angle radius = 1.5cm] {angle = otr--joint--base};
                
                  
                
                 


                
            \end{tikzpicture}

        \end{adjustbox}
    \end{center}
    \caption{A schematic of the beam profile monitoring system. \textbf{FIX LABELS + ORIENTATION}}
    \label{fig:profile_monitor}
\end{figure}
